Look-Ahead SCOPF (LASCOPF) for Tracking Demand Variation via Auxiliary Proximal Message Passing (APMP) Algorithm

In this paper, we will consider the Look-Ahead Security Constrained Optimal Power Flow (LASCOPF) problem looking forward multiple dispatch intervals, in which the load demand varies over dispatch intervals according to some forecast. We will consider the base-case and several contingency scenarios in the upcoming as well as in the subsequent dispatch intervals. We will formulate and solve the problem in a Model Predictive Control (MPC) paradigm. We will present the Auxiliary Proximal Message Passing (APMP) algorithm to solve this problem, which is a bi-layered decomposition-coordination type distributed algorithm, consisting of an outer Auxiliary Problem Principle (APP) layer and an inner Proximal Message Passing (PMP) layer. The APP part of the algorithm distributes the computation across several dispatch intervals and the PMP part performs the distributed computation within each of the dispatch interval across different devices (i.e. generators, transmission lines, loads) and nodes or nets. We will demonstrate the effectiveness of our method with a series of numerical simulations.

==> defs1.tex <==
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}

\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}

\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}

\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}

\newcommand{\sign}{\mathop{\bf sign}}
\newcommand{\devices}{\mathcal{D}}
\newcommand{\terminals}{\mathcal{T}}
\newcommand{\nets}{\mathcal{N}}
\newcommand{\AC}{\mathcal{T}^\mathrm{ac}}
\newcommand{\DC}{\mathcal{T}^\mathrm{dc}}
\DeclareMathOperator*{\cart}{\times}


==> message_passing.tex <==
\subsection{Message passing algorithm}

In this section, we describe the message passing algorithm used to solve
the SC-OPF. We begin by assuming that all device objective functions are
convex, closed, and proper (CCP) functions. We then derive a
distributed, message passing algorithm using operator splitting and the
alternating directions method of multipliers (ADMM) \cite{BP:11}. This
algorithm has guaranteed convergence for CCP functions, is fully
decentralized, is self-healing and robust, and is effectively
plug-and-play for security-constrained OPF problems.

\subsection{Consensus form SC-OPF}
Before applying ADMM to solve the SC-OPF, we first replicate the power
plans $P \in \reals^{|\terminals| \times (|\mathcal{L}|+1)}$ by introducing a copy,
$z \in \reals^{|\terminals| \times (|\mathcal{L}|+1)}$, of the plans. We then solve
the \emph{consensus form SC-OPF}:
\begin{equation}
\begin{array}{ll}
\mbox{minimize} & f(P) \\
\mbox{subject to} & \bar z = 0 \\
& P = z,
\end{array}
\end{equation} \label{p-consensus-scopf}

where $\bar z$ is the arithmetic mean of $z$ associated with a particular net. Because of the consensus constraint, when we solve the consensus form
SC-OPF, the optimal solution will agree with the solution of the
original SC-OPF. We introduce the indicator function $g(z) =
\mathcal{I}_{ \{ z \mid \bar z = 0 \}}(z)$, which is $0$ whenever $\bar
z = 0$ and $+\infty$ otherwise (if the power balance constraint is
violated). Because $\bar z$ is the average power at each net, the set
$\{ z \mid \bar z = 0 \}$ can be written as $\bigcap_{N_i \in \nets} \{ z
\mid \bar z_{N_i} = 0 \}$, where $\bar z_{N_i}$ is the average power at net $N_i$;
then,
\[
g(z) = \sum_{{N_i} \in \nets} g_{N_i}(z) = \sum_{{N_i} \in \nets} \mathcal{I}_{\{ z \mid \bar z_{N_i} = 0 \}}(z).
\]
Since the summands in the last expression only involve each net ${N_i}$
separately, $g(z)$ separates across nets completely
\[
g(z) = \sum_{{N_i} \in \nets} \mathcal{I}_{\{z_{N_i} \mid \bar z_{N_i} = 0\}} (z_{N_i}).
\]

\subsection{ADMM and the prox-project message passing algorithm}
We apply ADMM to solve the SC-OPF by
first forming the (scaled) augmented Lagrangian,
\[
\mathcal{L}(P,z,u) = f(P) + g(z) + (\rho/2)\|P - z + u\|_2^2,
\]
where $u = (1/\rho)y$ is the scaled dual variable $y$ associated with
the consensus constraint $p = z$. We obtained the augmented Lagrangian
by completing the squares.

ADMM is then
\BEAS
P^{(\nu+1)} & := & \argmin_{P} \left(f(P) + (\rho/2)\|P - z^{(\nu)} + u^{(\nu)}\|_2^2 \right)\\
z^{(\nu+1)} & := & \argmin_{z} \left(g(z) + (\rho/2)\|P^{(\nu+1)} - z + u^{(\nu)}\|_2^2 \right)\\
u^{(\nu+1)} & := & u^{(\nu)} + (P^{(\nu+1)} - z^{(\nu+1)}).
\EEAS
Note that the superscript is an iteration counter---not the contingency
label.

Because of our problem structure, we can further simplify ADMM. The
$P$-updates separate across devices and
\BEAS
P_d^{(\nu+1)} & := & \argmin_{P_d} \left(f_d(P_d) + (\rho/2)\|P_d - z_d^{(\nu)} + u_d^{(\nu)} \|_2^2\right)
\EEAS
%for all $d \in \devices$. Furthermore, the $z$-updates separate across
%nets and
%\BEAS
%z_{N_i}^{(\nu+1)}  :=  \argmin_{z_{N_i}} \left(\mathcal{I}_{\{z_{N_i} \mid \bar z_{N_i} = 0\}} (z_{N_i}) + (\rho/2)\|P_{N_i}^{(\nu+1)} - z_{N_i} + u_{N_i}^{(\nu)}\|_2^2\right)
%\EEAS
%for all ${N_i} \in \nets$. The $z_{N_i}$-update is just a Euclidean projection
%on to the set $\bar z_{N_i} = 0$ and can be solved analytically, so
%\BEAS
%z_{N_i}^{(\nu+1)} & := & P_{N_i}^{(\nu+1)} + u_{N_i}^{(\nu)} - \bar P_{N_i}^{(\nu+1)} - \bar u_{N_i}^{(\nu)}.
%\EEAS
for all $d \in \devices$. Furthermore, the $z$-updates separate across
nets and $z_{N_i}$-update is just a Euclidean projection
on to the set $\bar z_{N_i} = 0$ and can be solved analytically, so
\BEAS
z_{N_i}^{(\nu+1)} & = & P_{N_i}^{(\nu+1)} + u_{N_i}^{(\nu)} - \bar P_{N_i}^{(\nu+1)} - \bar u_{N_i}^{(\nu)}.
\EEAS
Substituting this expression for $z_{N_i}$ in to the $u$-update---which also
splits across nets---we obtain the \textbf{prox-project message passing
algorithm}:
\begin{enumerate}
\item \emph{Proximal plan updates.}
\BEAS
P_d^{(\nu+1)} & := &  \mathbf{prox}_{f_d,\rho}(P_d^{(\nu)} -\bar{P}_d^{(\nu)} - u_d^{(\nu)}),
\quad \forall d \in \devices.
\EEAS
\item \emph{Scaled price updates.}
\BEAS
u_{N_i}^{(\nu+1)} &:=& u_{N_i}^{(\nu)} + \bar P_{N_i}^{(\nu+1)}, \quad \forall {N_i} \in \nets,
\EEAS
\end{enumerate}
where the proximal function for a function $g$ is given by
\[
\mathbf{prox}_{g,\rho}(v) = \argmin_x (g(x) + (\rho/2)\|x - v\|_2^2).
\]
This algorithm alternates between evaluating prox functions (in
parallel) on each device and performing price updates on each net.
This algorithm has the following three properties:

\paragraph{Convergence.}
Since our prox-project message passing algorithm is a (simplified)
version of ADMM, the convergence results for ADMM also apply to
prox-project message passing. In particular, with mild conditions on
device objective functions $f_d$---namely, that they are closed, convex,
and proper---and provided a feasible solution exists, the following
properties of our algorithm hold.
\begin{enumerate}
\item \textit{Residual convergence.} $\bar P^{(\nu)} \to 0$ as $\nu \to \infty$,
\item \textit{Objective convergence.} $\sum_{d \in \devices} f_d(P_d^{(\nu)}) + \sum_{{N_i} \in \nets} g_{N_i}(P_{N_i}^{(\nu)}) \to f^\star$ as $\nu \to \infty$,
\item \textit{Dual variable convergence.} $\rho u^{(\nu)} = y^{(\nu)} \to y^\star$ as $\nu \to \infty$,
\end{enumerate}
where $f^\star$ is the optimal value for the (convex) SC-OPF, and
$y^\star$ are the optimal dual variables (prices). A proof of these
conditions can be found in \cite{BP:11}.

Convergence of our algorithm guarantees that, if message passing is run
long enough, power balance will be satisfied by $P^{(\nu)}$. Furthermore, this
$P^{(\nu)}$ will minimize the total cost of operating the network and, as a
byproduct, we also obtain variable contingency pricing.

\paragraph{Distributed.} Note that while the scaled price updates were
separated across nets, it could have also been separated across devices.
As long as each device has the ability to access the average power
imbalance for the nets it shares with its neighbors, this algorithm can
be completely decentralized. The scaled price updates can happen
locally, with each device retaining a copy of the (scaled) prices $u$.
This means that net computation (scaled price update) can be virtualized
and done on each device instead of on each net, as long as devices that
share a net are able to compute their average power imbalance. Then, the
algorithm consists of each device planning for each contingency and a
broadcast of plans to its neighbors. 
% The following observation follows from the fact that u_{n_1} = u_{n_2} = ... = u_{n_|n|}, but we did not establish that fact yet
%Alternatively, a price exchange can be used as a parity check for the algorithm.

\paragraph{Self-healing.} Because the semantics of a net is to enforce
power balance, when a device connects or disconnects from a net (\ie,
when the network topology changes), the algorithm can continue to
function without modification.

When the topology of the network changes, the current iterates $P^{(\nu)}$ and
$u^{(\nu)}$ of our algorithm can be used as a \emph{warm start}. Assuming
topology changes are not too frequent, the message passing algorithm
will simply converge to the new fixed point.

\subsection{Stopping criterion}We can define primal and dual residuals for the
prox-project message passing algorithm:
\[
r^{(\nu)} = \bar P^{(\nu)},
s^{(\nu)} = \rho\left((P^{(\nu)} - \bar P^{(\nu)}) - (P^{(\nu-1)} - \bar P^{(\nu-1)})\right).
\]
The
interpretation of $P^{(\nu)}$ is as a power plan.

A simple terminating criterion for prox-project message passing is when
\[
\| r^{(\nu)} \|_2 \leq \epsilon^\mathrm{pri}, \qquad \|s^{(\nu)}\|_2 \leq \epsilon^\mathrm{dual},
\]
where $\epsilon^\mathrm{pri}$ and $\epsilon^\mathrm{dual}$ are,
respectively, primal and dual tolerances. We can normalize both of these
quantities to the network size by the relation
\[
\epsilon^\mathrm{pri} = \epsilon^\mathrm{dual} = \epsilon^\mathrm{abs} \sqrt{|\terminals|(|\mathcal{L}|+1)},
\]
for some absolute tolerance $\epsilon^\mathrm{abs} > 0$.

\subsection{Choice of $\rho$}
The value of the algorithm parameter $\rho$ can greatly affect the
convergence rate of the message passing algorithm. There are no known
methods for choosing the optimal value of $\rho$ \emph{a priori}, except
in certain special cases \cite{GT:12}.

Empirically, however, it has been observed that the choice of $\rho$
affects the convergence rate of the primal and dual residuals. If $\rho$
is too large, the dual residuals converge slowly. If $\rho$ is too
small, the primal residuals converge slowly. The optimal $\rho$ balances
the convergence rate of both residuals. From this observation, several
heuristics can be devised to modify $\rho$ at each iteration such that
the primal and dual residuals remain approximately the same size.

For more details on $\rho$ selection, consult \cite{BP:11,KC:13}.

\subsection{Implementation of proximal functions}
Each device is responsible for implementing its proximal function. In
general, evaluating the proximal function requires solving an
optimization problem. The complexity of solving this optimization
problem depends on the structure of the local problem. In the case of
SC-OPF, the variables are the local power plans $P_d$ and any other
private variables. At most, the variables are coupled through the base
case $P_d^{(0)}$. This results in an arrow structure in the KKT system
of the local optimization problem. This kind of structure can be
exploited and solved with linear complexity. If the power plans do not
couple through the base case, then the local problem is completely
separable across the contingencies.

Because of this simple structure in the local SC-OPF problems on each
device, we can quickly and efficiently evaluate the proximal functions
for each device.

